Distributed Matrix Completion and Robust Factorization

If learning methods are to scale to the massive sizes of modern datasets, it is essential for the field of machine learning to embrace parallel and distributed computing. Inspired by the recent development of matrix factorization methods with rich theory but poor computational complexity and by the relative ease of mapping matrices onto distributed architectures, we introduce a scalable divide-and-conquer framework for noisy matrix factorization. We present a thorough theoretical analysis of this framework in which we characterize the statistical errors introduced by the "divide" step and control their magnitude in the "conquer" step, so that the overall algorithm enjoys high-probability estimation guarantees comparable to those of its base algorithm. We also present experiments in collaborative filtering and video background modeling that demonstrate the near-linear to superlinear speed-ups attainable with this approach.

==> dfc-journal/theory-nystrom-noiseless.tex <==

\subsection{Noiseless MC}
We now present the proof of Thm.~\ref{thm:prob-exact},
which characterizes the ability of the generalized \nys method to
recover a target matrix exactly when $\M$ has low rank and low coherence.  In
what follows, we let $r = \rank{\M}$ and note that $\M$ admits a decomposition
$\M = \Y^{\top}\Z$ for some matrices $\Y\in\reals^{r\times m}$ and
$\Z\in\reals^{r\times n}$.  In particular, we let $\Y^{\top} =
\U_{M}\mSigma_{M}^{\half}$ and $\Z = \mSigma_{M}^{\half}\V_{M}^{\top}$, where
$\U_{M}\mSigma_{M}\V_{M}^{\top}$ is the compact SVD of $\M$.  By block
partitioning $\Y$ and $\Z$ as $\Y = \begin{bmatrix}\Y_1 & \Y_2\end{bmatrix}$
and $\Z = \begin{bmatrix}\Z_1 & \Z_2\end{bmatrix}$ for $\Y_1\in\reals^{r\times
d}$ and $\Z_1\in\reals^{r\times l}$, we may write $\W = \Y_1^{\top}\Z_1, \C =
\Y^{\top}\Z_1,$ and $\R = \Y_1^{\top}\Z$.

Prop.~\ref{prop:exact} shows that, like the \nys method~\cite{KumarMoTa09}, the
generalized \nys method yields exact recovery of $\M$ whenever $\rank{\M} =
\rank{\W}$.  The same result is established in~\citet{WangDoToLiGu09} with a
different proof.
\begin{proposition}
	\label{prop:exact}
	%
	Suppose $r = \rank{\M} \leq \min(d,l)$ and $\rank{\W} = r$.
	Then $\M = \Mgnys$.
\end{proposition}
\begin{proof}
By appealing to our factorized block decomposition, we may rewrite the
generalized \nys approximation as
\begin{equation*} 
%
\Mgnys = \C\W^+\R = \Y^{\top}\Z_1(\Y_1^{\top}\Z_1)^+\Y_1^{\top}\Z.
\end{equation*}
We first note that 
%
%
$\rank{\W}=r$ implies that $\rank{\Y_1}=r$ and
$\rank{\Z_1}=r$ so that $\Z_1\Z_1^{\top}$ and $\Y_1\Y_1^{\top}$ are full-rank.
Hence,
	$$(\Y_1^{\top}\Z_1)^+ = \Z_1^{\top}(\Z_1\Z_1^{\top})^{-1}(\Y_1\Y_1^{\top})^{-1}\Y_1,$$
	yielding
\begin{align*}
	\Mgnys & =
\Y^{\top}\Z_1\Z_1^{\top}(\Z_1\Z_1^{\top})^{-1}(\Y_1\Y_1^{\top})^{-1}\Y_1\Y_1^{\top}\Z
\\
&= \Y^{\top}\Z = \M.
\end{align*}
\end{proof}

Prop.~\ref{prop:exact} allows us to lower bound the probability of
exact recovery with the probability of randomly selecting a rank-$r$
submatrix.  As $\rank{\W}=r$ iff both $\rank{\Y_1}=r$ and $\rank{\Z_1}=r$, 
it suffices to characterize the probability of selecting full rank
submatrices of $\Y$ and $\Z$.

Following the treatment of the \nys method in~\citet{TalwalkarRo10}, we note
that $\mSigma_{M}^{-\half}\Z = \V_{M}^{\top}$ and hence that
$\Z_1^{\top}\mSigma_{M}^{-\half} = \V_{M,l}$ where
$\V_{M,l}\in\reals^{l\times r}$ contains the first $l$ components of the leading
$r$ right singular vectors of $\M$.  It follows that $\rank{\Z_1} =
\rank{\Z_1^{\top}\mSigma_{M}^{-\half}} = \rank{\V_{M,l}} =
\rank{\V_{M,l}^{\top}\V_{M,l}}$.  Similarly, $\rank{\Y_1} =
\rank{\U_{M,d}^{\top}\U_{M,d}}$ where $\U_{M,d}\in\reals^{d\times r}$
contains the first $d$ components of the leading $r$ left singular vectors of
$\M$. Thus, we have 
\begin{align}
	\label{eq:rankprobZ}
	&\Parg{\rank{\Z_1}=r} = \Parg{\rank{\V_{M,l}^{\top}\V_{M,l}}=r} \\
	\label{eq:rankprobY}
	&\Parg{\rank{\Y_1}=r} = \Parg{\rank{\U_{M,d}^{\top}\U_{M,d}}=r}.
\end{align}

Further, as in~\citet{TalwalkarRo10}, we can lower bound the RHSs of  
\eqref{eq:rankprobZ} and \eqref{eq:rankprobY} via
\begin{align}
	\label{eq:normprobV}
	&\Parg{\rank{\V_{M,l}^{\top}\V_{M,l}}=r} \geq
\Parg{\norm{c_1\V_{M,l}^{\top}\V_{M,l}-\I}_2<1} \\
	\label{eq:normprobU}
	&\Parg{\rank{\U_{M,d}^{\top}\U_{M,d}}=r} \geq
\Parg{\norm{c_2\U_{M,d}^{\top}\U_{M,d}-\I}_2<1}\, ,
\end{align}
for any $c_1, c_2 > 0$.  Thm.~\ref{thm:cohere}, a restatement of Thm.~2
of~\citet{TalwalkarRo10} using the inequality $\mu^2(\cdot) \le r \mu_0(\cdot)$,
provides conditions under which the RHSs of \eqref{eq:normprobV} and
\eqref{eq:normprobU} are large.  
\begin{theorem}[Thm.~2 of~\citet{TalwalkarRo10}]
	\label{thm:cohere}
	Define $\V \in \reals^{n\times r}$ such that $\V^{\top}\V=\I$ and let
	$\V_{l} \in \reals^{l\times r}$ be generated from $\V$ by sampling rows
	uniformly at random.  Then, for any $l$ that satisfies
	$l\geq \sampcoh(r,\mu_0(\V),\delta)$
the following holds with probability
	at least $1-\delta$,
	$$\norm{\frac{n}{l}\V_{l}^{\top}\V_{l} - \I}_2 < \half.$$
\end{theorem}


We can now prove Thm.~\ref{thm:prob-exact}.
  Let $d\geq \sampcoh(r, \mu_0(\U_M), 1-\sqrt{1-\delta})$ and $l\geq\sampcoh(r, \mu_0(\V_M),  
  1-\sqrt{1-\delta})$ as specified in Thm.~\ref{thm:prob-exact}.
  Then, by Thm.~\ref{thm:cohere} and \eqref{eq:normprobV} and \eqref{eq:normprobU},
  \begin{align*}
		\sqrt{1-\delta} &\leq \Parg{\norm{\frac{m}{d}\U_{M,d}^{\top}\U_{M,d} - \I}_2
< \half} \\
& \leq \Parg{\norm{\frac{m}{d}\U_{M,d}^{\top}\U_{M,d} - \I}_2 < 1} \\
& \leq \Parg{\rank{\U_{M,d}^{\top}\U_{M,d}} = r} \\
  \end{align*}
  and
  \begin{align*}
		\sqrt{1-\delta} & \leq \Parg{\norm{\frac{n}{l}\V_{M,l}^{\top}\V_{M,l} - \I}_2
< \half} \\
& \leq \Parg{\norm{\frac{n}{l}\V_{M,l}^{\top}\V_{M,l} - \I}_2 < 1} \\
& \leq \Parg{\rank{\V_{M,l}^{\top}\V_{M,l}} = r}.
  \end{align*}
  Furthermore, by the independence of row and column sampling 
  and \eqref{eq:rankprobZ} and \eqref{eq:rankprobY}, we see that
\begin{align*}
	1-\delta & \leq \Parg{\rank{\U_{M,d}^{\top}\U_{M,d}} =
r}\Parg{\rank{\V_{M,l}^{\top}\V_{M,l}} = r} \\ 
&  = \Parg{\rank{\Y_1} = r}\Parg{\rank{\Z_1} = r} \\
& = \Parg{\rank{\W}=r}.
\end{align*}
  Finally, Prop.~\ref{prop:exact} implies that
  $$\Parg{\M = \Mgnys} \geq \Parg{\rank{\W}=r}\geq 1-\delta,$$
  which proves the statement of the theorem.

